BirdSet: A Large-Scale Dataset for Audio Classification in Avian Bioacoustics

Deep learning (DL) has greatly advanced audio classification, yet the field is limited by the scarcity of large-scale benchmark datasets that have propelled progress in other domains. While AudioSet is a pivotal step to bridge this gap as a universal-domain dataset, its restricted accessibility and limited range of evaluation use cases challenge its role as the sole resource. Therefore, we introduce BirdSet, a large-scale benchmark dataset for audio classification focusing on avian bioacoustics. BirdSet surpasses AudioSet with over 6,800 recording hours ($\uparrow\!17\%$) from nearly 10,000 classes ($\uparrow\!18\times$) for training and more than 400 hours ($\uparrow\!7\times$) across eight strongly labeled evaluation datasets. It serves as a versatile resource for use cases such as multi-label classification, covariate shift or self-supervised learning. We benchmark six well-known DL models in multi-label classification across three distinct training scenarios and outline further evaluation use cases in audio classification. We host our dataset on Hugging Face for easy accessibility and offer an extensive codebase to reproduce our results.

==> tables/deprecated/related_datasets.tex <==
\renewcommand{\arraystretch}{0.8} % Increase row height
\begin{tabular}{m{4cm}lccccc@{\hspace{0.3cm}}cccccccccc}
\toprule
    % && \multicolumn{5}{c}{\textbf{\focalunderline{Focals \icon{figures/focalsymbol.pdf}}}}  & \multicolumn{10}{c}{\textbf{\scapeunderline{Soundscapes \iconsmall{figures/soundscapesymbol.pdf}}}} \\
      && \multicolumn{5}{c}{\textbf{{{Focals}}}}  & \multicolumn{10}{c}{\textbf{{Soundscapes}}} \\
          \cmidrule(lr){3-7}
    \cmidrule(lr){8-17}
    % && \multicolumn{3}{c}{\textbf{Focals}} & \multicolumn{10}{c}{\textbf{Soundscapes}} & \multicolumn{3}{c}{\textbf{???}} \\
    & & \textsc{\textbf{XC}}         & \textsc{\textbf{INA}}      & \textsc{\textbf{MAC}}   & \textsc{\textbf{CBI}} & \textsc{\textbf{BD}} & \textsc{\textbf{HSN}}     & \textsc{\textbf{SNE}}      & \textsc{\textbf{UHH}}     & \textsc{\textbf{PER}}    & \textsc{\textbf{SSW}}    & \textsc{\textbf{POW}} & \textsc{\textbf{CAP}} & \textsc{\textbf{NBP}}  & \textsc{\textbf{S2L}}  & \textsc{\textbf{VOX}}  \\
    \midrule
  
       \multirow{2}{*}{{\textbf{\citet{bellafkir2023}}}}& {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes  \\
    & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no  \\
    \hline
        

    \multirow{2}{*}{{\textbf{\citet{bellafkir2024}}}} & {train} & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval}  & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no  \\

    % \hline
    %    \multirow{2}{*}{{\textbf{\citet{bicudo2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
    % & {eval} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes \\
    
        \hline
       \multirow{2}{*}{{\textbf{\citet{bravosanchez2021}}}} & {train} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no  \\
    & {eval} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no  \\

   \hline
       \multirow{2}{*}{{\textbf{\citet{clark2023}}}} & {train} & \yes & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no\\
    \hline

        \multirow{2}{*}{{\textbf{\citet{denton2021}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes   \\
    & {eval}  & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \yes & \no & \yes &  \no &  \no &  \no  \\
    \hline

       \multirow{2}{*}{{\textbf{\citet{eichinski2022}}}} & {train} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\

   \hline
       \multirow{2}{*}{{\textbf{\citet{fu2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\

    % \hline
    %    \multirow{2}{*}{{\textbf{\citet{ghani2023}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
    % & {eval} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\

     \hline
       \multirow{2}{*}{{\textbf{\citet{gupta2021}}}} & {train} & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval} & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    \hline
    \multirow{2}{*}{{\textbf{\citet{hamer2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes   \\
    & {eval}  & \no & \no & \no & \no & \no & \yes & \yes & \yes & \yes & \yes & \yes & \yes &  \no &  \no &  \no    \\
\hline
       \multirow{2}{*}{{\textbf{\citet{hoechst22}}}} & {train} & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval} & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\

    \hline
       \multirow{2}{*}{{\textbf{\citet{hu2023_lightweight}}}} & {train} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no \\
    & {eval} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\

   \hline
       \multirow{2}{*}{{\textbf{\citet{hu2023a}}}} & {train} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no \\
    & {eval} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no\\

   \hline
       \multirow{2}{*}{{\textbf{\citet{jeantet2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    \hline
          \multirow{2}{*}{{\textbf{\citet{kahl2021}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes  \\
    & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no  \\

   

   \hline
       \multirow{2}{*}{{\textbf{\citet{liu2022_ensemble}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\

   \hline
   \multirow{2}{*}{{\textbf{\citet{liu2022_channelfusion}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\
    & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no   \\

   \hline
       \multirow{2}{*}{{\textbf{\citet{swaminathan2024}}}} & 
       {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
    & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no   \\


   \hline
       \multirow{2}{*}{{\textbf{\citet{tang2023}}}} & 
       {train} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no   \\
    & {eval}  & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no   \\
    
   \hline
       \multirow{2}{*}{{\textbf{\citet{wang2022}}}} & 
       {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no   \\
    & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no \\

   \hline
       \multirow{2}{*}{{\textbf{\citet{xiao2022}}}} & 
       {train} & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
    & {eval}  & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
    
       \hline
       \multirow{2}{*}{{\textbf{\citet{xie2022}}}} & 
       {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
    & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\

   \hline
       \multirow{2}{*}{{\textbf{\citet{zhang2023_representation}}}} & 
       {train} & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
    & {eval}  & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
   % \hline
   %     \multirow{2}{*}{{\textbf{\citet{zhang2023_fusion_transformer}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
   %  & {eval} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
\midrule
    \multirow{2}{*}{\small{\texttt{BirdSet}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes   \\
    & {eval}  & \no & \no & \no &  \no & \no & \yes & \yes & \yes & \yes & \yes & \yes & \no &  \yes &  \no &  \no  \\

\bottomrule
\end{tabular}


% \renewcommand{\arraystretch}{0.55} % Increase row height
% \begin{tabular}{llccccc@{\hspace{0.3cm}}cccccccccc@{\hspace{0.3cm}}cc}
% \toprule
%     % && \multicolumn{5}{c}{\textbf{\focalunderline{Focals \icon{figures/focalsymbol.pdf}}}}  & \multicolumn{10}{c}{\textbf{\scapeunderline{Soundscapes \iconsmall{figures/soundscapesymbol.pdf}}}} \\
%       && \multicolumn{5}{c}{\textbf{{{Focals}}}}  & \multicolumn{10}{c}{\textbf{{Soundscapes}}} \\
%           \cmidrule(lr){3-7}
%     \cmidrule(lr){8-17}
%     % && \multicolumn{3}{c}{\textbf{Focals}} & \multicolumn{10}{c}{\textbf{Soundscapes}} & \multicolumn{3}{c}{\textbf{???}} \\
%     & & \textsc{\textbf{XC}}         & \textsc{\textbf{INA}}      & \textsc{\textbf{MAC}}   & \textsc{\textbf{CBI}} & \textsc{\textbf{BD}} & \textsc{\textbf{HSN}}     & \textsc{\textbf{SNE}}      & \textsc{\textbf{UHH}}     & \textsc{\textbf{PER}}    & \textsc{\textbf{SSW}}    & \textsc{\textbf{POW}} & \textsc{\textbf{CAP}} & \textsc{\textbf{NBP}}  & \textsc{\textbf{S2L}}  & \textsc{\textbf{VOX}} & \textsc{\deemph{\textbf{UC}*}} \\
%     \midrule
  
%        \multirow{2}{*}{{\textbf{\citet{bellafkir2023}}}}& {train}* & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes &\no \\
%     & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &\no \\
%         \hline

%     \multirow{2}{*}{{\textbf{\citet{bellafkir2024}}}} & {train} & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no &\yes \\
%     & {eval}  & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &\yes \\

%     % \hline
%     %    \multirow{2}{*}{{\textbf{\citet{bicudo2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
%     % & {eval} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes \\
    
%         \hline
%        \multirow{2}{*}{{\textbf{\citet{bravosanchez2021}}}} & {train} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no \\
%     & {eval} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no \\

%    \hline
%        \multirow{2}{*}{{\textbf{\citet{clark2023}}}} & {train} & \yes & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
%     & {eval} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no\\
%     \hline

%        \multirow{2}{*}{{\textbf{\citet{eichinski2022}}}} & {train} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes \\
%     & {eval} & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes \\

%    \hline
%        \multirow{2}{*}{{\textbf{\citet{fu2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
%     & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\

%     % \hline
%     %    \multirow{2}{*}{{\textbf{\citet{ghani2023}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
%     % & {eval} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\

%      \hline
%        \multirow{2}{*}{{\textbf{\citet{gupta2021}}}} & {train} & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
%     & {eval} & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\

%     \hline

%        \multirow{2}{*}{{\textbf{\citet{hoechst22}}}} & {train} & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes \\
%     & {eval} & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes \\

%     \hline
%        \multirow{2}{*}{{\textbf{\citet{hu2023_lightweight}}}} & {train} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no \\
%     & {eval} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no  \\

%    \hline
%        \multirow{2}{*}{{\textbf{\citet{hu2023a}}}} & {train} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no \\
%     & {eval} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no  \\

%    \hline
%        \multirow{2}{*}{{\textbf{\citet{jeantet2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no \\
%     & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no \\


%    \hline
%        \multirow{2}{*}{{\textbf{\citet{liu2022_ensemble}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
%     & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\

%    \hline
%    \multirow{2}{*}{{\textbf{\citet{liu2022_channelfusion}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
%     & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no  \\

%    % \hline
%    % \multirow{2}{*}{{\textbf{\citet{lu2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
%    %  & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\
    
%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{manzano-rubio2022}}}} & {train} & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no &  \no \\
%    %  & {eval}  & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \yes \\
%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{muhling2022}}}} & {train} & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no&  \no \\
%    %  & {eval}  & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no &  \yes&  \no&  \no \\

%    % \hline ONLY BIRDNET
%    %     \multirow{2}{*}{{\textbf{\citet{nolan2023}}}} & 
%    %     {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
%    %  & {eval}  & \no & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no \\ 

%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{noumida2023}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
%    %  & {eval} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\

%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{provost2022}}}} & 
%    %     {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \no  \\
%    %  & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \no \\

%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{puget}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
%    %  & {eval} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\

%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{stein2023}}}} & 
%    %     {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \no  \\
%    %  & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \no \\

%    \hline
%        \multirow{2}{*}{{\textbf{\citet{swaminathan2024}}}} & 
%        {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \no   \\
%     & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \no   \\


%    \hline
%        \multirow{2}{*}{{\textbf{\citet{tang2023}}}} & 
%        {train} & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \no   \\
%     & {eval}  & \yes & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no & \no   \\
    
%    \hline
%        \multirow{2}{*}{{\textbf{\citet{wang2022}}}} & 
%        {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
%     & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no &  \no\\

%    \hline
%        \multirow{2}{*}{{\textbf{\citet{xiao2022}}}} & 
%        {train} & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no  \\
%     & {eval}  & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no  \\
    
%        \hline
%        \multirow{2}{*}{{\textbf{\citet{xie2022}}}} & 
%        {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no  \\
%     & {eval}  & \yes & \no & \no & \no & \no & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no  \\

%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{yan2021}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
%    %  & {eval} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\

%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{yang2022}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
%    %  & {eval} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\

%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{xiao2022}}}} & 
%    %     {train} & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\
%    %  & {eval}  & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no  \\

%    \hline
%        \multirow{2}{*}{{\textbf{\citet{zhang2023_representation}}}} & 
%        {train} & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no  \\
%     & {eval}  & \no & \no & \no & \no & \yes & \no & \no & \no & \no &  \no &  \no &  \no &  \no &  \no &  \no&  \no  \\
%    % \hline
%    %     \multirow{2}{*}{{\textbf{\citet{zhang2023_fusion_transformer}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
%    %  & {eval} & \yes & \no & \yes & \no & \no & \no & \no & \yes & \no & ... & ... & ... & ... & ... & ... & ... \\
% \midrule
%     \multirow{2}{*}{{\textbf{\citet{denton2021}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes  &\no \\
%     & {eval}  & \no & \no & \no & \no & \no & \yes & \yes & \yes & \yes & \yes & \yes & \yes &  \no &  \no &  \no   &\no \\
%     \hline
    
%     \multirow{2}{*}{{\textbf{\citet{hamer2023}}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes  &\no \\
%     & {eval}  & \no & \no & \no & \no & \no & \yes & \yes & \yes & \yes & \yes & \yes & \yes &  \no &  \no &  \no   &\no \\
    
%     \hline
%        \multirow{2}{*}{{\textbf{\citet{kahl2021}}}} & {train} & \yes & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \yes \\
%     & {eval} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \yes  \\

%    \hline
%     \multirow{2}{*}{{\texttt{BirdSet}}} & {train} & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes&  \no   \\
%     & {eval}  & \no & \no & \no &  \no & \no & \yes & \yes & \yes & \yes & \yes & \yes & \no &  \yes &  \no &  \no&  \no   \\

% \bottomrule
% \end{tabular}

==> tables/deprecated/related_models.tex <==



\renewcommand{\arraystretch}{1} % Increase row height
\begin{tabular}{l 
                c c %@{\hspace{0.2cm}}
                cc %@{\hspace{0.1cm}}
                cc 
                }
       \toprule
    \rule{0pt}{-5cm}& \multicolumn{2}{c}{\textbf{Task}} 
    & \multicolumn{2}{c}{\textbf{Model}}  
    & \multicolumn{2}{c}{\textbf{Input}} 
     \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5} \cmidrule(lr){6-7} 
    
    \rule{0pt}{-1cm}& \iconmed{figures/multilabel_symbol.pdf} &  \iconmed{figures/multiclass_symbol.pdf}
    & \multicolumn{1}{c}{CNN} & \multicolumn{1}{c}{Transf.} 
    & Spec & Wave 
    \\
    \midrule
    \scriptsize{\textbf{\cite{bellafkir2023}}} &\yes & \no & \yes  & \no & \yes &\no \\
    \hline
    \scriptsize{\textbf{\cite{bellafkir2024}}} & \yes & \no & \no  & \yes & \yes & \no  \\
    \hline
    \scriptsize{\textbf{\cite{bravosanchez2021}}} & \no & \yes & \yes  & \no & \no & \yes \\
    \hline
    \scriptsize{\textbf{\cite{clark2023}}}  & \yes & \no & \yes  & \no & \yes & \no \\
     \hline
         \scriptsize{\textbf{\cite{denton2021}}} & \yes &\no& \yes  & \no & \yes & \no \\
     \hline
    \scriptsize{\textbf{\cite{eichinski2022}}} & \no &\yes & \yes  & \no & \yes & \no \\
     \hline
    \scriptsize{\textbf{\cite{fu2023}}} & \yes &\no & \yes  & \no & \yes & \no \\
     \hline
    \scriptsize{\textbf{\cite{gupta2021}}} & \no &\yes & \yes  & \no & \yes & \no \\
     \hline
         \scriptsize{\textbf{\cite{hamer2023}}} & \yes & \no & \yes  & \no & \yes & \no \\
     \hline
    \scriptsize{\textbf{\cite{hoechst22}}} & \yes & \no & \yes  & \no & \yes & \no \\
     \hline
    \scriptsize{\textbf{\cite{hu2023_lightweight}}} & \no & \yes & \yes  & \no & \yes & \no \\
    \hline
   \scriptsize{\textbf{\cite{hu2023a}}} & \no & \yes & \yes & \no & \yes & \no \\
     \hline
    \scriptsize{\textbf{\cite{jeantet2023}}} & \no & \yes & \yes  & \no & \yes  & \no \\
      \hline
    \scriptsize{\textbf{\cite{kahl2021}}} & \yes &\no& \yes & \no & \yes & \no \\
     \hline
    \scriptsize{\textbf{\cite{liu2022_ensemble}}} & \no & \yes & \yes  & \no & \yes & \no \\
      \hline
   \scriptsize{\textbf{\cite{liu2022_channelfusion}}} & \no & \yes & \yes  & \no & \yes & \no \\
     \hline
   \scriptsize{\textbf{\cite{swaminathan2024}}}  & \yes & \no & \no  & \yes & \no & \yes \\
     \hline
   \scriptsize{\textbf{\cite{tang2023}}} & \no & \yes & \no  & \yes & \yes & \no\\
     \hline
   \scriptsize{\textbf{\cite{wang2022}}} & \no &\yes & \no  & \no & \yes & \no  \\
     \hline
   \scriptsize{\textbf{\cite{xiao2022}}} & \no & \yes & \yes  & \no & \yes & \no \\
     \hline
   \scriptsize{\textbf{\cite{xie2022}}} & \no & \yes & \yes  & \no & \yes & \no \\
     \hline
   \scriptsize{\textbf{\cite{zhang2023_representation}}} & \no &\yes& \yes   & \no & \yes & \no \\
        \midrule
   \scriptsize{\texttt{BirdSet}} & \yes & \no & \yes  & \yes & \yes & \yes \\
   \bottomrule
\end{tabular}

